Reading Human Preference from Looped Transformer Internal States

Show a frozen language model two replies to the same request, one of which a person preferred. Can a small probe on the model's hidden states tell which? On Ouro-2.6B-Thinking, a model that runs its layers four times per token, and Anthropic's HH-RLHF data, the answer is yes, but only faintly. A linear probe picks the preferred reply 61.5% of the time, a small nonlinear network that scores each reply separately 64.9%, and the evaluator trained for version 1 reaches 64.7% on the test split: clearly better than simple rules such as picking the longer reply, but weak. Whether preference is stored as a comparison between the two replies or as a property of each is still open. A linear probe cannot tell, and a network that reads both replies together has an estimated edge of only 0.7 points (95% CI 0.0 to 1.4) over one that scores each reply separately. These numbers hold under three controls: scoring every pair in both orders, splitting the data by pair, and, for the probes, keeping the end of each conversation, where the two replies differ. Version 1's 95.2% and 84.5% were obtained without the first two and do not hold; version 2's corrected relational-probe accuracy, obtained without the third, was four to five points too low. This version replaces both.

==> paper_style/boxes.tex <==
\tcbset{
  kirinbase/.style={
    enhanced,
    breakable,
    boxrule=0.55pt,
    arc=2.5mm,
    outer arc=2.5mm,
    left=3.2mm,right=3.2mm,top=2.4mm,bottom=2.4mm,
    before skip=6pt,after skip=7pt,
    fonttitle=\sffamily\bfseries,
    coltitle=KirinInk,
    coltext=KirinInk
  }
}

\newtcolorbox{abstractbox}{
  kirinbase,
  title=Abstract,
  colback=white,
  colbacktitle=white,
  coltitle=KirinAccentDark,
  colframe=KirinAccent,
  borderline north={1.0pt}{0pt}{KirinAccent},
  fontupper=\small,
  before upper={\setlength{\parindent}{1em}}
}

% Companion to abstractbox for the page-2 "Results at a glance" layer: same
% framing, no title — the section heading inside the box carries the name.
\newtcolorbox{glancebox}{
  kirinbase,
  colback=white,
  colframe=KirinAccent,
  borderline north={1.0pt}{0pt}{KirinAccent},
  fontupper=\small,
  before upper={\setlength{\parindent}{1em}}
}

\newtcolorbox{resultbox}[1][Result]{
  kirinbase,title=#1,
  colback=KirinAccentFaint,
  colbacktitle=KirinAccentPale,
  coltitle=KirinAccentDark,
  colframe=KirinAccent,
  borderline west={2.2pt}{0pt}{KirinAccent}
}

\newtcolorbox{scopebox}[1][]{
  kirinbase,
  title=#1,
  colback=KirinAccentFaint,
  colframe=KirinRule,
  borderline west={1.6pt}{0pt}{KirinAccent},
  fontupper=\small
}

\newtcolorbox{auditbox}[1][Audit note]{
  kirinbase,title=#1,
  colback=KirinAccentFaint,
  colbacktitle=KirinAccentPale,
  coltitle=KirinUnresolved,
  colframe=KirinUnresolved,
  borderline west={2.2pt}{0pt}{KirinUnresolved}
}

\newtcolorbox{roadmapbox}[1][How to read this paper]{
  kirinbase,title=#1,
  colback=white,
  colbacktitle=white,
  coltitle=KirinAccentDark,
  colframe=KirinRule,
  borderline north={1.0pt}{0pt}{KirinAccent},
  fontupper=\small
}

% Pandoc block quotes become restrained scope/proposition boxes.
\renewenvironment{quote}{\begin{scopebox}}{\end{scopebox}}


==> paper_style/palette.tex <==
\definecolor{KirinInk}{HTML}{172027}
\definecolor{KirinMuted}{HTML}{52606A}
\definecolor{KirinRule}{HTML}{D6DDE1}
\definecolor{KirinBaseline}{HTML}{7D858C}
\definecolor{KirinPositive}{HTML}{16756A}
\definecolor{KirinUnresolved}{HTML}{8F6400}
\definecolor{KirinNegative}{HTML}{A94442}
\definecolor{KirinLink}{HTML}{2E4A75}

\ifkirinmethodology
  \definecolor{KirinAccent}{HTML}{B85C1E}
  \definecolor{KirinAccentDark}{HTML}{874319}
  \definecolor{KirinAccentPale}{HTML}{FBF0E6}
  \definecolor{KirinAccentFaint}{HTML}{FDF8F3}
\else
  \definecolor{KirinAccent}{HTML}{3A5683}
  \definecolor{KirinAccentDark}{HTML}{263C63}
  \definecolor{KirinAccentPale}{HTML}{EDF1F7}
  \definecolor{KirinAccentFaint}{HTML}{F7F9FC}
\fi
\color{KirinInk}



==> paper_style/tables.tex <==
\sisetup{
  detect-all,
  input-open-uncertainty=,
  input-close-uncertainty=,
  table-number-alignment=center,
  group-separator={,},
  group-minimum-digits=4
}

\setlength{\tabcolsep}{4.5pt}
\renewcommand{\arraystretch}{1.12}
\arrayrulecolor{KirinRule}
\AtBeginEnvironment{longtable}{%
  \small
  \setlength{\tabcolsep}{4pt}%
  \renewcommand{\arraystretch}{1.10}%
}
\AtBeginEnvironment{tabular}{\small}
\setlength{\LTpre}{5pt}
\setlength{\LTpost}{6pt}
\setlength{\heavyrulewidth}{0.8pt}
\setlength{\lightrulewidth}{0.45pt}
\setlength{\cmidrulewidth}{0.35pt}
\newcommand{\kirintablehead}[1]{\rowcolor{KirinAccentPale}\sffamily\bfseries #1}
\newcommand{\statusEstablished}{\textsc{Established}}
\newcommand{\statusBounded}{\textsc{Bounded screen}}
\newcommand{\statusUnresolved}{\textsc{Unresolved}}
\newcommand{\statusDiagnostic}{\textsc{Diagnostic}}
\newcommand{\statusRetracted}{\textsc{Retracted}}
\newcommand{\statusHistorical}{\textsc{Historical}}
\newcommand{\statusCorrected}{\textsc{Corrected}}



==> paper_style/titlepage.tex <==
\newcommand{\KirinTitleBlock}[7]{%
  \thispagestyle{fancy}%
  \begingroup
  \setlength{\parindent}{0pt}%
  \noindent\begin{minipage}[t]{0.72\linewidth}
    {\sffamily\bfseries\fontsize{8.5pt}{10pt}\selectfont\color{KirinAccent}\MakeUppercase{#1}}
  \end{minipage}%
  \begin{minipage}[t]{0.28\linewidth}
    \raggedleft{\sffamily\fontsize{8.5pt}{10pt}\selectfont\color{KirinMuted}#6}
  \end{minipage}\par
  \vspace{4pt}\color{KirinAccent}\hrule height 0.85pt\color{KirinInk}\vspace{9pt}
  {\sffamily\bfseries\fontsize{23pt}{25.2pt}\selectfont\raggedright #2\par}
  \vspace{4pt}
  {\sffamily\fontsize{15.2pt}{17.5pt}\selectfont\color{KirinAccentDark}\raggedright #3\par}
  \vspace{8pt}\color{KirinRule}\hrule height 0.45pt\color{KirinInk}\vspace{7pt}
  {\sffamily\bfseries\fontsize{11.5pt}{13.2pt}\selectfont #4}\par
  \vspace{2pt}
  {\sffamily\fontsize{8.9pt}{10.6pt}\selectfont\color{KirinMuted}%
    \href{https://github.com/VykosMolt}{github.com/VykosMolt}%
    \enspace\textcolor{KirinRule}{|}\enspace
    \href{https://github.com/VykosMolt/Hidden-State-Evaluator}{github.com/VykosMolt/Hidden-State-Evaluator}%
    \ifstrempty{#5}{}{\enspace\textcolor{KirinRule}{|}\enspace #5}%
  }\par
  \ifstrempty{#7}{}{\vspace{5pt}{\sffamily\fontsize{8.5pt}{10.2pt}\selectfont\color{KirinMuted}#7\par}}
  \vspace{6pt}
  \endgroup
}

\newenvironment{kirinacknowledgment}{%
  \par\vspace{1pt}\begingroup\small\setlength{\parindent}{0pt}%
  \noindent\textbf{Acknowledgments.}\enspace
}{%
  \par\endgroup\vspace{4pt}%
}

